Polar and Convolutional Codes for the Unequal Message Protection Problem

This paper proposes the design of polar and convolutional coset codes for the unequal message protection (UMP) in the short blocklength regime, to overcome the rate loss introduced by preamble-based solutions. After providing conditions to ensure message class disjointness, a two-step decoding architecture is proposed: it first identifies the message class via a likelihood ratio test--computable exactly for convolutional codes and approximated for polar codes--and subsequently performs maximum (or near) likelihood decoding among the codewords of the chosen message class. Numerical results show that our construction closely tracks finite-length benchmarks. Specifically, the analyzed CRC-aided polar codes perform comparable to existing polar code approaches, without requiring specific code design, while offering a robust and spectrally efficient solution for UMP scenarios.

==> sections/conclusions.tex <==
\section{Conclusions}\label{sec:conclusions}


==> sections/intro.tex <==
\section{Introduction}\label{sec:intro}


==> sections/preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminaries}
%\subsection{Notation}\label{suc:notation}

